Fine-Grained Lineage for Safer Notebook Interactions

Computational notebooks have emerged as the platform of choice for data science and analytical workflows, enabling rapid iteration and exploration. By keeping intermediate program state in memory and segmenting units of execution into so-called "cells", notebooks allow users to execute their workflows interactively and enjoy particularly tight feedback. However, as cells are added, removed, reordered, and rerun, this hidden intermediate state accumulates in a way that is not necessarily correlated with the notebook's visible code, making execution behavior difficult to reason about, and leading to errors and lack of reproducibility. We present NBSafety, a custom Jupyter kernel that uses runtime tracing and static analysis to automatically manage lineage associated with cell execution and global notebook state. NBSafety detects and prevents errors that users make during unaided notebook interactions, all while preserving the flexibility of existing notebook semantics. We evaluate NBSafety's ability to prevent erroneous interactions by replaying and analyzing 666 real notebook sessions. Of these, NBSafety identified 117 sessions with potential safety errors, and in the remaining 549 sessions, the cells that NBSafety identified as resolving safety issues were more than $7\times$ more likely to be selected by users for re-execution compared to a random baseline, even though the users were not using NBSafety and were therefore not influenced by its suggestions.

==> algofix.tex <==
%ref: https://tex.stackexchange.com/questions/195991/aligning-in-and-out-text-for-algorithms

\makeatletter
\renewcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2}\algocf@typo:}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\everypar={\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
  }}%
\makeatother


==> cell-example.tex <==
\begin{figure}[t]
\begin{lstjupyter}[cellsidebar=refresh,cellnum=1]{In1}
 def!
   \tikz[remember picture] \node [] (a) {};
 !puissance(x, n):
     i = !\HL!p = 1!\HL!
     a = b + 1
     for (i in !\HL!range(n)!\HL!):
         p = p * x!\tikz[remember picture] \node [inner xsep = 0pt] (b){};!
     print("hi")
     return p!
       \tikz[remember picture] \node [] (c){};!
\end{lstjupyter}
\begin{tikzpicture}[remember picture, overlay,
    every edge/.append style = { ->, thick, >=stealth,
                                  gray, dashed, line width = 1pt },
    every node/.append style = { align = center, minimum height = 10pt,
                                 font = \scriptsize\bfseries, fill= green!20},
                  text width = 2.5cm ]
  \node [above right = 0.5cm and -0.5cm of a, text width = 1.9cm] (A) {function name};
  \node [right = 1.9cm of b]  (B) {instructions};
  \node [right = 2.cm of c]  (C) {instruction \texttt{\bfseries return}};  
  \draw (A.south) + (0, 0) coordinate(x2) edge (x2|-a.north);
  \draw (B.west) edge (b.east) ;  
  \draw (C.west) edge (c.east) ;
  %\connectzm{In1-1}{blue}
  %\connectzm{In1-2}{purple}
\end{tikzpicture}

\begin{lstjupyter}[celltype=output,cellsidebar=unsafe,cellnum=1]{Out1}
 "ERROR: unable to !\HL!define!\HL! function !\HL!puissance!\HL!"
\end{lstjupyter}
\vspace{-1em}
\caption{Example sequence of notebook interactions leading to counterintuitive behavior.}
\label{fig:intro-interactions}
\end{figure}

==> scalable-lineage-example.tex <==
\begin{figure}[t]
\begin{lstjupyter}[cellnum=1]{sc1}
  x = 0
  for i in range(10**7):
      x += lst[i]
\end{lstjupyter}

%\begin{lstjupyter}[cellnum=2]{sc2}
%\end{lstjupyter}
%\begin{tikzpicture}[remember picture, overlay]
%\tikzset{myarrow/.style={->, >=latex', shorten >=1pt, thick}}
%\end{tikzpicture}
\vspace{2em}
\caption{$\parents{x} = \verb!lst[0]!$ after the cell executes, since
\name only instruments each statement the first time it executes in order
to strike a tradeoff between correctness and performance.}
\label{fig:scalable-lineage-example}
\end{figure}

==> vldbreffix.tex <==
\usepackage{textcase}

\makeatletter
\def\@sect#1#2#3#4#5#6[#7]#8{%
    \ifnum #2>\c@secnumdepth
        \let\@svsec\@empty
    \else
        \refstepcounter{#1}%
        \edef\@svsec{%
            \begingroup
                %\ifnum#2>2 \noexpand\rm \fi % changed to next 29 July 2002 gkmt
                        \ifnum#2>2 \noexpand#6 \fi
                \csname the#1\endcsname
            \endgroup
            \ifnum #2=1\relax .\fi
            \hskip 1em
        }%
    \fi
    \@tempskipa #5\relax
    \ifdim \@tempskipa>\z@
        \begingroup
            #6\relax
            \@hangfrom{\hskip #3\relax\@svsec}%
            \begingroup
                \interlinepenalty \@M
                \if@uchead
                    \MakeTextUppercase{#8}% HERE
                \else
                    #8%
                \fi
                \par
            \endgroup
        \endgroup
        \csname #1mark\endcsname{#7}%
        \vskip -12pt  %gkmt, 11 aug 99 and GM July 2000 (was -14) - numbered section head spacing
\addcontentsline{toc}{#1}{%
            \ifnum #2>\c@secnumdepth \else
                \protect\numberline{\csname the#1\endcsname}%
            \fi
            #7%
        }%
    \else
        \def\@svsechd{%
            #6%
            \hskip #3\relax
            \@svsec
            \if@uchead
                \uppercase{#8}%
            \else
                #8%
            \fi
            \csname #1mark\endcsname{#7}%
            \addcontentsline{toc}{#1}{%
                \ifnum #2>\c@secnumdepth \else
                    \protect\numberline{\csname the#1\endcsname}%
                \fi
                #7%
            }%
        }%
    \fi
    \@xsect{#5}\hskip 1pt
    \par
}
\makeatother



==> workflow-highlight-nohighlight.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\begin{minipage}{0.4\linewidth}
\begin{lstjupyter}[cellnum={[1]},cellnumoffs=-7mm]{wfhl1}
 def ...
     ...
\end{lstjupyter}
\makesecondcellmarker{wfhl1}{4}

%\begin{lstjupyter}[cellnum=2]{wfhl2}
%\begin{lstjupyter}[cellnum={[2]},cellnumoffs=-7mm]{wfhl2}
\begin{lstjupyter}[cellnum={[2]},highlight=refresh,cellnumoffs=-7mm]{wfhl2}
 agg_by_col = ...
\end{lstjupyter}

%\begin{lstjupyter}[cellnum=3]{wfhl3}
%\begin{lstjupyter}[cellnum={[3]},cellnumoffs=-7mm]{wfhl3}
\begin{lstjupyter}[cellnum={[3]},highlight=unsafe,cellnumoffs=-7mm]{wfhl3}
 df_x_agg = ...
 df_y_agg = ...
\end{lstjupyter}
\begin{tikzpicture}[remember picture, overlay]
\tikzset{myarrow/.style={->, >=latex', shorten >=1pt, thick}}
\draw[myarrow,->] (wfhl1-cell-marker.south) to [out=90,in=90] (wfhl2-cell-marker.north);
\draw[myarrow,->] (wfhl2-cell-marker.south) to [out=90,in=90] (wfhl3-cell-marker.north);
\draw[myarrow,->] ([shift={(1mm,0)}]wfhl3-cell-marker.north) to [out=45,in=-90] ([shift={(0mm,0)}]wfhl1-second-marker.south);
\end{tikzpicture}
\end{minipage}
&
\begin{minipage}{0.4\linewidth}
\begin{lstjupyter}[cellnum={[1]}]{wfnohl1}
 def custom...
     ...
\end{lstjupyter}

\begin{lstjupyter}[cellnum={[2]}]{wfnohl2}
 agg_by_col = ...
\end{lstjupyter}

\begin{lstjupyter}[cellnum={[3]}]{wfnohl3}
 df_x_agg = ...
 df_y_agg = ...
\end{lstjupyter}
\begin{tikzpicture}[remember picture, overlay]
\tikzset{myarrow/.style={->, >=latex', shorten >=1pt, thick}}
\draw[myarrow,->] (wfnohl1-cell-marker.south) to (wfnohl2-cell-marker.north);
\draw[myarrow,->] (wfnohl2-cell-marker.south) to (wfnohl3-cell-marker.north);
\end{tikzpicture}
\end{minipage}
\end{tabular}
\end{center}
\vspace{2em}
\end{figure}

